Online Grounding of Symbolic Planning Domains in Unknown Environments

If a robotic agent wants to exploit symbolic planning techniques to achieve some goal, it must be able to properly ground an abstract planning domain in the environment in which it operates. However, if the environment is initially unknown by the agent, the agent needs to explore it and discover the salient aspects of the environment needed to reach its goals. Namely, the agent has to discover: (i) the objects present in the environment, (ii) the properties of these objects and their relations, and finally (iii) how abstract actions can be successfully executed. The paper proposes a framework that aims to accomplish the aforementioned perspective for an agent that perceives the environment partially and subjectively, through real value sensors (e.g., GPS, and on-board camera) and can operate in the environment through low level actuators (e.g., move forward of 20 cm). We evaluate the proposed architecture in photo-realistic simulated environments, where the sensors are RGB-D on-board camera, GPS and compass, and low level actions include movements, grasping/releasing objects, and manipulating objects. The agent is placed in an unknown environment and asked to find objects of a certain type, place an object on top of another, close or open an object of a certain type. We compare our approach with the state of the art methods on object goal navigation based on reinforcement learning, showing better performances.

==> figures/framework.tex <==
\begin{figure}[h]

\scalebox{0.85}{

 \begin{tikzpicture} 
     \definecolor{mycyan}{RGB}{0, 102, 102}
     \definecolor{myorange}{RGB}{204, 102, 0}
     \definecolor{mygreen}{RGB}{87, 253, 115}
     \tikzstyle{arrow} = [thick,->,>=stealth]
     \tikzstyle{point} = [circle,fill=black, minimum size=1.5mm, inner sep=0pt, text width=1mm]

 \node (environment) [outer sep=0, draw, rectangle,
     fill=mygreen!20, minimum width=8cm, minimum height=1.1cm,
     scale=.8]{$E=(\S,\mathcal{E},\gamma)$};
     
     
 \node (knowledge_builder) [outer sep=0, draw, rectangle,
     fill=mygreen!20, minimum width=3cm, minimum height=1.1cm,
     scale=.8, above = of environment]{update agent
       belief state};
     
 \node (belief_state) [outer sep=0, draw, ellipse, fill=mygreen!20,
     minimum width=3cm, minimum height=1.1cm, scale=.8, above = of
     knowledge_builder]{$\C',\ Pr(\bm Y_{\C'})$};
          
 \node (symbolic_planner) [outer sep=0, draw, rectangle,
     fill=cyan!20, minimum width=3cm, minimum height=1.1cm, scale=.8,
     above = of belief_state]{Symbolic planner};

 \node (controller_planner) [outer sep=0, draw, rectangle,
     fill=cyan!20, minimum width=3cm, minimum height=1.1cm, scale=.8,
     right = of belief_state]{$\exec(a)$};
     
 \node (action_model) [outer sep=0, draw, rectangle, fill=cyan!20,
     minimum width=3cm, minimum height=1.1cm, scale=.8, left= of
     belief_state]{$\delta$ of $\actmodel(\C')$};
     
\node (symbolic_goal) [above = of symbolic_planner]{Planning domain $\actmodel$, symbolic goal};

 \node (constraints) [outer sep=0, draw, ellipse, fill=cyan!20,
     minimum width=3cm, minimum height=1.1cm, scale=.8, below = of
     action_model]{State constraints};
     
 \draw [arrow] (environment) -- node[left]{$\bm x$} (knowledge_builder);
     
     \draw [arrow] (constraints)  -- (knowledge_builder);
     
     \draw [arrow] (belief_state) -- node[left]{$\bm y'$} (symbolic_planner);
     
     \draw [arrow] (symbolic_goal) -- (symbolic_planner);
     
     \draw [arrow] (symbolic_planner) -- node[sloped,above]{$a$} (controller_planner);
     
     \draw [arrow] (controller_planner) to[bend left = 10] node[right]{$e$} (environment);
     
     \draw [arrow] (environment.east) to[bend right] node[right]{$feed_e$} (controller_planner);
     
     \draw [arrow] (action_model) -- node[below,sloped]{$\delta(\bm y', a)$} (knowledge_builder);

     \draw [arrow] (symbolic_planner) to node[above,sloped]{$a$} (action_model);
     
     \draw [arrow] (belief_state) to node[above,sloped]{$\bm y', \bm z'$} (controller_planner);
     
     \draw [arrow] (belief_state) to node[above,sloped]{$\bm y'$} (action_model);

     \draw [arrow, <->] (belief_state) to node[left]{$\bm Z_{\C'}$} (knowledge_builder);

    %  \draw [arrow] (belief_state) to[bend left] (knowledge_builder);
     
    %  \draw [arrow] (knowledge_builder) to[bend left] (belief_state);
     
     \draw [arrow] (controller_planner) -- node[sloped,above]{success} node[sloped,below]{fail} (knowledge_builder);
     
     \draw [arrow] (symbolic_goal) to[bend right] node[above,sloped]{$\actmodel$} (action_model);
     \end{tikzpicture}
     }
     
     
     
 \end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> figures/object_detector.tex <==

 
 \begin{figure}
\centering
\begin{subfigure}{.5\columnwidth}
  \centering
  \includegraphics[width=.85\linewidth]{figures/object_detector/object_detector_recall_IoU50_alldet100.jpg}
  \caption{Test Recall.}
  \label{fig:sub1}
\end{subfigure}%
\begin{subfigure}{.5\columnwidth}
  \centering
  \includegraphics[width=.85\linewidth]{figures/object_detector/object_detector_precision_IoU50_alldet100.jpg}
  \caption{Test Precision.}
  \label{fig:sub2}
\end{subfigure}
\caption{Evaluation metrics of the Faster-RCNN object detector computed with IoU 50\% over all (100) detections.}
\label{fig:test}
\end{figure}

==> figures/ogn_metrics_evolution_ithor.tex <==

 \begin{figure}[t]
\centering
\includegraphics[width=.95\linewidth]{figures/ogn_metrics_evolution_ithor.png}
\caption{Average metrics of the goal object navigation tasks over 200 steps in the iTHOR simulator.}
\label{fig:ogn_metrics_evolution_ithor}
\end{figure}

==> figures/on_predicate_classifier.tex <==

 
 \begin{figure}
\centering
\begin{subfigure}{.5\columnwidth}
  \centering
  \includegraphics[width=.85\linewidth]{figures/on_predicate_classifier/on_test_acc.jpg}
  \caption{Test accuracy}
  \label{fig:sub1}
\end{subfigure}%
\begin{subfigure}{.5\columnwidth}
  \centering
  \includegraphics[width=.85\linewidth]{figures/on_predicate_classifier/on_test_fscore.jpg}
  \caption{Test F-measure}
  \label{fig:sub2}
\end{subfigure}
\caption{Evaluation metrics of the ``on(object1, object2)" predicate classifier.}
\label{fig:test}
\end{figure}

==> figures/robothor_ogn_fails_classes.tex <==
 \begin{figure}
\centering
\includegraphics[width=.95\linewidth]{figures/ogn_failures_classes.png}
\caption{Failure of the goal object navigation task in the RoboTHOR simulator, aggregated by goal object types.}
\label{fig:ogn_metrics_evolution}
\end{figure}

==> sections/03_problem.tex <==
\section{Problem}
\todo[inline]{Descrizione del problema che vogliamo risolvere. Da decidere se inglobarlo nell’introduzione (x limiti di spazio)
An agent in an unseen environment, is positioned randomly in the position and it has to perform some high level task, as object goal navigation, changing the status of an object (open/close), or moving object one on top of the other.
This problem is some intermediate problem between object goal navigation and rearrangement. We want to show that with a single architecture we can solve multiple problems.}

==> tables/OLD_OLD_OLD_all_tasks.tex <==
\begin{table}[t]

\textcolor{red}{
\centering
\setlength{\tabcolsep}{3pt}
\scalebox{0.74}{
 \begin{tabular}{l c c | c c | c c | c c | c c | c c} 
 \hline
  & \multicolumn{2}{c |}{Success} & \multicolumn{2}{c |}{DTS} & \multicolumn{2}{c |}{P$_{objs}$} & \multicolumn{2}{c |}{R$_{objs}$} & \multicolumn{2}{c |}{P$_{pred}$} & \multicolumn{2}{c |}{R$_{pred}$} \\ 
  & $\alg$ & $GT$ & $\alg$ & $GT$ & $\alg$ & $GT$ & $\alg$ & $GT$ & $\alg$ & $GT$ & $\alg$ & $GT$ \\ 
 \hline\hline
 \textsc{On} & 0.46 & 0.63 & 0.94 & 0.62 & 0.3 & 1 & 0.85 & 1 & 0.74 & 0.72 & 0.83 & 0.88 \\ 
 \textsc{Open} & 0.5 & 0.68 & 0.77 & 0.47 & 0.38 & 1 & 0.76 & 1 & 0.75 & 0.72 & 0.73 & 0.84 \\ 
 \textsc{Close} & 0.67 & 0.81 & 0.61 & 0.29 & 0.39 & 1 & 0.73 & 1 & 0.73 & 0.73 & 0.71 & 0.84 \\ 
 \hline
 \end{tabular}
 }
 \caption{\textcolor{red}{OLD RESULTS} Our model evaluated on the tasks of opening/closing an object and placing an object on another one for 56, 52 and 100 episodes respectively. We compare the performances without and with the ground truth object detections.}
 }
\end{table}

==> tables/OLD_OLD_all_tasks.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{3pt}
\scalebox{0.74}{

\textcolor{red}{
 \begin{tabular}{l c c | c c | c c | c c | c c | c c} 
 \hline
  & \multicolumn{2}{c |}{\emph{Success}} & \multicolumn{2}{c |}{\emph{DTS}} & \multicolumn{2}{c |}{$P_{\C}$} & \multicolumn{2}{c |}{$R_{\C}$} & \multicolumn{2}{c |}{$P_{\bm Y_{\C}^{GT}}$} & \multicolumn{2}{c |}{$R_{\bm Y_{\C}^{GT}}$} \\ 
  & $\C$ & $\C_{GT}$ & $\C$ & $\C_{GT}$ & $\C$ & $\C_{GT}$ & $\C$ & $\C_{GT}$ & $\C$ & $\C_{GT}$ & $\C$ & $\C_{GT}$ \\ 
 \hline\hline
 \textsc{On} & 0.4 & 0.63 & 1.13 & 0.73 & 0.31 & 1 & 0.83 & 1 & 0.83 & 0.83 & 0.75 & 0.83 \\ 
 \textsc{Open} & 0.55 & 0.64 & 0.74 & 0.51 & 0.4 & 1 & 0.76 & 1 & 0.85 & 0.83 & 0.66 & 0.77 \\
 \textsc{Close} & 0.81 & 0.94 & 0.31 & 0.07 & 0.39 & 1 & 0.75 & 1 & 0.84 & 0.82 & 0.63 & 0.73 \\
 \hline
 \end{tabular}
 }
 }
 \caption{\textcolor{red}{OLD RESULTS} Our model evaluated on the tasks of opening/closing an object and placing an object on another one for 56, 52 and 100 episodes respectively. We compare the performances without and with the ground truth object detections $\C_{GT}$.}
\end{table}

==> tables/OLD_all_tasks.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{3pt}
\scalebox{0.74}{
\textcolor{red}{
 \begin{tabular}{l c c | c c | c c | c c | c c | c c} 
 \hline
  & \multicolumn{2}{c |}{\emph{Success}} & \multicolumn{2}{c |}{\emph{DTS}} & \multicolumn{2}{c |}{$P_{\C}$} & \multicolumn{2}{c |}{$R_{\C}$} & \multicolumn{2}{c |}{$P_{\bm Y_{\C}^{GT}}$} & \multicolumn{2}{c |}{$R_{\bm Y_{\C}^{GT}}$} \\ 
  & $\C$ & $\C_{GT}$ & $\C$ & $\C_{GT}$ & $\C$ & $\C_{GT}$ & $\C$ & $\C_{GT}$ & $\C$ & $\C_{GT}$ & $\C$ & $\C_{GT}$ \\ 
 \hline\hline
 \textsc{On} & 0.51 & - & 0.87 & - & 0.29 & 1 & 0.85 & 1 & 0.84 & - & 0.79 & - \\ 
 \textsc{Open} & 0.75 & - & 0.5 & - & 0.36 & 1 & 0.79 & 1 & 0.84 & - & 0.72 & - \\
 \textsc{Close} & 0.86 & - & 0.2 & - & 0.34 & 1 & 0.79 & 1 & 0.82 & - & 0.71 & - \\
 \hline
 \end{tabular}
 }
 }
 \caption{\textcolor{red}{OLD RESULTS} Our model evaluated on the tasks of opening/closing an object and placing an object on another one for 56, 52 and 100 episodes respectively. We compare the performances without and with the ground truth object detections $\C_{GT}$.}
\end{table}

==> tables/task_ogn_mini.tex <==
\begin{table}[t]
\centering
\scalebox{0.9}{
 \begin{tabular}{l c c c} 
 \hline
  & Success & SPL & DTS \\ 
 \hline\hline
 \arch$_{200_{step}}$ & 0.42 & 0.19 & 2.2 \\ 
 \arch$_{GT}$ & - & - & -\\
 DD-PPO$_{200_{step}}$ & 0.32 & 0.16 & 2.16\\
 DD-PPO$_{500_{step}}$ & 0.38 & 0.17 & 2.09\\
 DD-PPO$_{action\_boost}$ & - & - & -\\
 \hline
 \end{tabular}
 }
 \caption{(225 EPISODI) Our model evaluated on the Object Goal Navigation task. We compare \arch\ w/o ground truth object detections, RL baselines and the winner of the Object Goal Navigation 2021 challenge in the RoboTHOR simulator.}
 \label{tab:robothor}
\end{table}
